Reasoning about Agent Programs using ATL-like Logics

We propose a variant of Alternating-time Temporal Logic (ATL) grounded in the agents' operational know-how, as defined by their libraries of abstract plans. Inspired by ATLES, a variant itself of ATL, it is possible in our logic to explicitly refer to "rational" strategies for agents developed under the Belief-Desire-Intention agent programming paradigm. This allows us to express and verify properties of BDI systems using ATL-type logical frameworks.

==> 6-conclusion.tex <==
\section{Discussion}\label{sec:conclusions}
\notem{1. Plans with multiple actions and subgoaling. 2. Combine achievement and maintenence goals.}

In this paper, we have developed an ATL-like logic that relates closely to the BDI agent-oriented programming paradigm that is widely used to \emph{implement} multi-agent systems.
%%
In the new logic, the user can express structures that represent the capability of BDI agents in a natural way and can reason in the language about what agents can achieve under such capabilities. 
%%
Although our framework is abstract and hence not linked to any \emph{specific} BDI programming framework, it is possible to prove  its relationship with most such languages under plausible assumptions (e.g., use of conjunctive goals only, linear execution model, etc.) 


Though not included for lack of space, a graphical representation of the technical notions used and a reduction of our logic to a version of ATLES with nondeterministic commitment functions can be found in~\cite{us-aaai11}. We shall include this content in the final version with an extra \nolinebreak page.

There are a number of assumptions made here that could be relaxed but that require further work.
%%
Since we have used the valuation function $\V$ in a structure, all the agents are assumed to have full observability of the environment. This is, of course, a strong assumption in many settings.
%%
Also, our logic allows us to reason about the rational behavior of an agent \emph{with an initial set of goals}. It would be interesting to extend it so that agents can adopt new goals when interacting with other agents (e.g., an agent agrees to achieve a goal on behalf of another agent).
%% 
Finally, we have assumed a linear style of execution for BDI programs, that is, agents work on one goal at a time. However, many BDI systems also allow for interleaved execution of different plans for different goals. To account for such execution model, one would only need to redefine set $\exec_\agt(\plan{},\Pi,g,\lambda^+)$.





We close the paper by noting that, besides ATLES of course, our work has strong similarities and motivations to those on \emph{plausibility} \cite{jamroga:AAMAS07} and \emph{intention}~\cite{jamroga:Springer2005} reasoning  in ATL. Like ATLES, however, those works are still not linked to any approach for the actual development of agents, which is the main motivation behind our work. Nonetheless, we would like to investigate how to integrate plausibility reasoning in our logic, as we believe it is orthogonal to that of rational BDI-style behavior. Indeed, the plausibility approach allows us to focus the reasoning to certain parts of an ATL structure using more declarative specifications.   


% 
% ks done earlier on plausibility, with plausibility in this setting be defined by the agent's capabilities. But, the frameworks that define \emph{plausibility}~\cite{jamroga:AAMAS07} and  require the strategies to be defined before hand.

==> alg-BDI-Eval.tex <==
\begin{algorithm}[t]
\textbf{function} \BDIEval($\M_{\varrho},\omega,\varrho,\mapCap,\coalition{A}\varphi$) returns $[\coalitione{A}{\varrho,\omega}\varphi]$ in $\M$

\Indp    \lCase{$\varphi = \mnext \theta:$}{
         $[\coalition{A}\varphi] = \Pre(A,\omega,\mapCap,[\theta]) $%\cap \llbracket \varrho \rrbracket$
    }
    \\
    \Case{$\varphi = \always \theta:$}{
         $\rho=[true]; \tau=[\theta]$ \;
           \lWhile{$\rho \not\subseteq \tau$}{$\rho=\tau; \tau = \Pre(A,\omega,\mapCap,\rho)\cap [\theta]$ \od} \\
         $[\coalition{A}\varphi]=\rho$ % \cap \llbracket \varrho \rrbracket$
    }
    
    \Case{$\varphi = \theta_1 \until \theta_2:$}{
           $\rho=[false]; \tau=[\theta_2]$ \;
           \lWhile{$\tau \not\subseteq \rho$}{$\rho=\rho \union \tau; \tau = \Pre(A,\omega,\mapCap,\rho) \cap [\theta_1]$ \od} \\
           $[\coalition{A}\varphi]=\rho$ % \cap \llbracket \varrho \rrbracket$
    }
\Indm    
\Return $\ws([\coalition{A}\varphi] \cap \llbracket \varrho \rrbracket)$
    
\caption{\BDIEval function}
\label{algo:BDI-Eval}
\end{algorithm}

